A 3D Generative Model for Structure-Based Drug Design

We study a fundamental problem in structure-based drug design -- generating molecules that bind to specific protein binding sites. While we have witnessed the great success of deep generative models in drug design, the existing methods are mostly string-based or graph-based. They are limited by the lack of spatial information and thus unable to be applied to structure-based design tasks. Particularly, such models have no or little knowledge of how molecules interact with their target proteins exactly in 3D space. In this paper, we propose a 3D generative model that generates molecules given a designated 3D protein binding site. Specifically, given a binding site as the 3D context, our model estimates the probability density of atom's occurrences in 3D space -- positions that are more likely to have atoms will be assigned higher probability. To generate 3D molecules, we propose an auto-regressive sampling scheme -- atoms are sampled sequentially from the learned distribution until there is no room for new atoms. Combined with this sampling scheme, our model can generate valid and diverse molecules, which could be applicable to various structure-based molecular design tasks such as molecule sampling and linker design. Experimental results demonstrate that molecules sampled from our model exhibit high binding affinity to specific targets and good drug properties such as drug-likeness even if the model is not explicitly optimized for them.

==> etc/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{} We will provide the complete codes and data once this paper is published.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/10-intro-backup.tex <==
\section{Introduction}
\label{sec:intro}

Designing molecules that bind to a specific protein binding site, also known as structure-based drug design, is one of the most challenging tasks in drug discovery \cite{anderson2003sbdd}.
Searching for suitable molecule candidates \textit{in silico} usually involves massive computational efforts because of the enormous space of synthetically feasible chemicals \cite{polishchuk2013estimation} and conformational degree of freedom of both compound and protein structures \cite{hawkins2017conformation}.

In recent years, we have witnessed the success of machine learning approaches to problems in drug design, especially on molecule generation.
Most of these approaches use deep generative models to propose drug candidates by learning the underlying distribution of molecules with desired properties.
However, most of such methods are generally SMILES/string-based \cite{gomezb2018automatic, kusner2017grammar} or graph-based \cite{li2018learning,liu2018constrained, jin2018junction, jin2020composing}, attempting to represent small molecular in a more compact low dimensional space.
Hence, these methods are not applicable to generating molecules that fit to a specific protein structure which is also known as the drug target.
To address this problem, researchers start to study how to design molecules directly in 3D space \cite{gebauer2019gschnet, simm2020molgym, simm2020molgymv2, masuda2020ligan}. Most of these methods \cite{gebauer2019gschnet, simm2020molgym, simm2020molgymv2} can only handle very small organic molecules (<9 atoms), which is not sufficient to generate drug-scale molecules which usually contain dozens of heavy atoms.
Another thread of work \cite{masuda2020ligan} proposes to generate voxelized molecular images and use a post-processing algorithm to reconstruct molecular structures.
Though this method could produce drug-scale molecules for specific protein pockets, the quality and diversity of the molecular is heavily limited by the voxelization techiques, which can only XXXXX.
Therefore, generating high-quality drug molecules for specific 3D protein binding sites remains challenging.

In this work, we propose a new generative model, named XXXX, to generate new drugs by modeling the distribution of atom occurrence in the 3D space of the protein binding site. 
Formally, given the 3D structure of the binding site $\gC$, we model the distribution $p(e, \vr | \gC)$, where $\vr \in \sR^3$ is an arbitrary 3D coordinate and $e$ is atom type.
We design a neural network architecture which takes as input a query 3D coordinate $\vr$, conditional on the 3D context $\gC$, and outputs the probability of $\vr$ being occupied by an atom of a particular chemical element.
In order to ensure the distribution is equivariant to $\gC$'s rotation and translation, we utilize graph neural networks to perceive the context of each query coordinate. 

Despite having a powerful neural network to model the distribution of atom occurrence $p(e, \vr | \gC)$, how to generate \textit{valid} and \textit{diverse} molecules is technically challenging for the following two reasons: 
First, simply drawing \textit{i.i.d.} samples from the distribution $p(e, \vr | \gC)$ does not yield valid molecules because atoms within a molecule are not independent of each other by forming various chemical bonds.
Second, a new sampling algorithm needs to be designed to capture the multi-modality of the feasible chemical space, i.e. it should be able to generate a diverse set of desired molecules given a specific binding context.

To tackle the challenge, we propose an auto-regressive sampling algorithm.
In specific, we start with a context consisting of only protein atoms. Then, we iteratively sample one atom from the distribution at each step and add it to the context to be used in the next step, until there is no room for new atoms.
Compared to other recent methods \cite{masuda2020ligan, ragoza2020gridgen}, our auto-regressive algorithm is much simpler and more advantageous since it does not rely on post-processing algorithms to infer atom placements from density. 
More importantly, it is capable of multi-modal sampling by the nature of auto-regressive and is able to avoid additional latent variables via VAEs \cite{kingma2013vae} or GANs \cite{goodfellow2014gans} which would bring about extra architectural complexity and training difficulty.

We conduct extensive experiments to evaluate our approach.
Quantitative and qualitative results show that:
(1) our method is able to generate diverse drug-like molecules that have high binding affinity to specific targets based on 3D structures of protein binding sites;
(2) our method is able to generate molecules with fairly high drug-likeness score (QED) \cite{bickerton2012qedscore} and synthetic accessibility score (SA) \cite{ertl2009sascore} even if the model is not specifically optimized for them;
(3) in addition to molecule generation, the proposed method is also applicable to other relevant tasks such as linker design.




==> tables/design-main-t.tex <==
\begin{tabular}{l | cc | cc | cc | cc}
\toprule
 & \multicolumn{2}{c|}{Vina Score} 
 & \multicolumn{2}{c|}{High Affinity} 
 & \multicolumn{2}{c|}{\multirow{2}{*}{QED ($\uparrow$)}} 
 & \multicolumn{2}{c}{\multirow{2}{*}{SA ($\uparrow$)}}  \\

 & \multicolumn{2}{c|}{(kcal/mol, $\downarrow$)} 
 & \multicolumn{2}{c|}{(\%, $\uparrow$)} &  &  \\

Method & Avg. & Med. & Avg. & Med. & Avg. & Med. & Avg. & Med. \\
\midrule

liGAN &  &  &  &  &  &  &  &  \\
Ours &  &  &  &  &  &  &  &  \\
Ref &  &  &  &  &  &  &  &  \\
\bottomrule
\end{tabular}

==> tables/linker-main-t.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
Model & \multicolumn{3}{c|}{$\text{SC}_\text{RDKit}$ Molecule (\%)} & \multicolumn{3}{c|}{$\text{SC}_\text{RDKit}$ Fragments (\%)} & \multicolumn{3}{c}{RMSD Fragments (\%)}\\
& > 0.7 & > 0.8 & > 0.9 & > 0.7 & > 0.8 & > 0.9 & < 1.00 (\AA) & < 0.75 (\AA) & < 0.50 (\AA) \\
\midrule
DeLinker &  59.17 & 20.00 & 0.00 & 75.83 & 33.33 & 5.83 & 75.00 & 39.17 & 14.17 \\
Ours & & & & & & & & & \\
\bottomrule
\end{tabular}
